Monarch: A Durable Polymorphic Memory For Data Intensive Applications

3D die stacking has often been proposed to build large-scale DRAM-based caches. Unfortunately, the power and performance overheads of DRAM limit the efficiency of high-bandwidth memories. Also, DRAM is facing serious scalability challenges that make alternative technologies more appealing. This paper examines Monarch, a resistive 3D stacked memory based on a novel reconfigurable crosspoint array called XAM. The XAM array is capable of switching between random access and content-addressable modes, which enables Monarch (i) to better utilize the in-package bandwidth and (ii) to satisfy both the random access memory and associative search requirements of various applications. Moreover, the Monarch controller ensures a given target lifetime for the resistive stack. Our simulation results on a set of parallel memory-intensive applications indicate that Monarch outperforms an ideal DRAM caching by 1.21x on average. For in-memory hash table and string matching workloads, Monarch improves performance up to 12x over the conventional high bandwidth memories.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> related.tex <==
\section{Related Work}

\paragraph{Non-Volatile Memories for database applications}
Past research in NVM for Hash Tables \cite{hashpcm, pathhash, levelhash} have been in building novel songlie-node hash table structures to benefit from the non-volatility and low latency of NVM.  This work proposes a new memristor based memory architecture, which can be exploited to optimize open addressing based single-node hash tables. HiKV \cite{hikv} focuses on designing an hash table which does hybrid indexing in hybrid memory such that it can exploit the fast index searching capability of NVM and fast read latency of DRAM. 

NVMcached \cite{nvmcached} designs an NVM based key-value cache using byte-addressable NVM for key-value store. They report a maximum throughput of 4.8x on YCSB workloads while Monarch achieves a maximum speedup of around 13x.

FaRM and HERD \cite{farm,herd} use Hopscotch Hashing in improving distributed systems hash table performance using RDMA. Monarch is focused on improving performance of single-node hash tables.

RC-NVM \cite{rcnvm} proposes a RRAM based architecture which supports row and column accesses to memory, which allows for optimizations for iMDB based applications like SQL. RC-NVM also proposes new instructions to enable row/column storage of data. XCache, unlike RC-NVM, exploits the search capability of the proposed 2R memristive cells for a different category of iMDB applications - Hash Tables. 

Li-Si Monola \cite{Zha2018} proposes a reconfigurable computing fabric coupled with RRAM based memory to alleviate FPGA performance and energy efficiency for diverse cloud workloads. 

\paragraph{High-Bandwidth Memories for database applications}

Research on stream processing on HBM has largely focused on comparing sort merge v/s hash join performance. StreamBox-HBM \cite{StreamBox} proposes a stream analytics engine optimized for HBM, where-in they find that sequential sort algorithms for grouping are better than hash based join algorithms for HBM. Monarch optimizes stream processing applications, and operates at the same maximum bandwidth as HBM.  

Recent work on optimizing HBMs for hash tables have focused on alleviating the overhead of pointer chasing  \cite{pointerchase}, which uses the logic layer of the HBM to perform some in memory comutations for pointer chasing, thereby alleviating the data transfer cost from CPU to memory. This provides optimization for hash tables with separate chaining based conflict resolution. While Monarch implicitly reduces data transfers from memory to CPU for Hash Table lookups, it focuses on hash tables with open addressing based conflict resolution, which requires no pointer chasing. 

\paragraph{High-Bandwidth Non-Volatile memory}

R-Cache \cite{rcache} proposes an highly set-associative, in-package cache made by 3D die stacking of memristive memory arrays. But R-Cache is purely hardware managed and has no reconfigurability, and the transaction flow differs between Monarch and R-Cache.

\paragraph{Software defined caches}

Sofware defined caches has been proposed previously by researchers. Jenga \cite{jenga} is such one work which builds virtual cache hierarchies depending on the needs of the OS. Banshee \cite{banshee}  exploits software hardware interplay by combining page-tabe based page mapping management adn badnwidth efficient cache replacement. Monarch provides configurability at a higher level, where the OS can dictate which part of the application needs to run with Monarch as cache, while it can configure a part of Monarch as software defined scratchpad and control data placement with the full address space of the scratchpad being visible.

\paragraph{Persistent Memories}

Intel Optane 3D XPoint features a crosspoint structure made of fast switching material. Optane DC \cite{optaneanalysis} supports Memory (cached) and App Direct (uncached) modes. In Memory mode it is used as cache for DDRx, which helps hide the drawbacks of the low bandwidth of DDRx, while in App Direct mode, it is used as a persistent storage device, similiar to Monarch. Optane has been shown to have almost 2x faster than their counterparts for file-system storages. However, Monarch is different due to it's multidimensional access and search capability.

\paragraph{Associative search based architectures}

Architectures which allow for associative search based on TCAMs have been proposed in the past for different applications \cite{agrawal1994fast, meribout2000using, guo2013ac, de2000needles, ranger2007evaluating}. Monarch is RRAM based and works at a much finer granularity than the previous works. The X-WideIO interface also allows for a much higher bandwidth than the previous works, an instance of which can be noted at the difference in performance of string match between Monarch and \cite{guo2013ac}.





 

==> xrotor.tex <==
\paragraph{X-Cache Wear Leveling.}

